Bipartite Stochastic Matching: Online, Random Order, and I.I.D. Models

Within the context of stochastic probing with commitment, we consider the online stochastic matching problem; that is, the one sided online bipartite matching problem where edges adjacent to an online node must be probed to determine if they exist, based on known edge probabilities. If a probed edge exists, it must be used in the matching (if possible). We study this problem in the generality of a patience (or budget) constraint which limits the number of probes that can be made to edges adjacent to an online node. The patience constraint results in modelling and computational efficiency issues that are not encountered in the special cases of unit patience and full (i.e., unlimited) patience. The stochastic matching problem leads to a variety of settings. Our main contribution is to provide a new LP relaxation and a unified approach for establishing new and improved competitive bounds in three different input model settings (namely, adversarial, random order, and known i.i.d.). In all these settings, the algorithm does not have any control on the ordering of the online nodes. We establish competitive bounds in these settings, all of which generalize the standard non-stochastic setting when edges do not need to be probed (i.e., exist with certainty). All of our competitive ratios hold for arbitrary edge probabilities and patience constraints: (1) A $1-1/e$ ratio when the stochastic graph is known, offline vertices are weighted and online arrivals are adversarial. (2) A $1-1/e$ ratio when the stochastic graph is known, edges are weighted, and online arrivals are given in random order (i.e., in ROM, the random order model). (3) A $1-1/e$ ratio when online arrivals are drawn i.i.d. from a known stochastic type graph and edges are weighted. (4) A (tight) $1/e$ ratio when the stochastic graph is unknown, edges are weighted and online arrivals are given in random order.

==> content/ROM-iid <==
\ABc{This is where the Karade et al proof goes showing ROM implies iid. We have to argue that this still works in the stochastic rewards setting.}


\ABc{What other (if any) classical results have to be stated and proved here?}
\label{app:ROM-iid}


==> content/benchmarks.tex <==
%\ARc{I think that we should combine this and the next section.}

In adversarial online competitive analysis, we compare the value of the matching returned by an online algorithm to that of an optimal matching. If the inputs are drawn from a distribution, then we compare the expected value of the matching returned by an online algorithm to the expected value of the optimal matching. For stochastic probing problems, it is easy to see we cannot hope to obtain a reasonable competitive bound for this comparison.
%if we are comparing the expected value of on online algorithm to the expectation of an optimal value obtained while knowing the instatiations of the given probabilities. 
For example, consider a single online vertex with partience 1, and $n$ offline (unweighted) vertices where each edge $e$ has probability $\frac{1}{n}$ of being present. The expectation of an online probing algorithm will be $\frac{1}{n}$ while the expectation (over all instantiations of the edge probabilities) will be $1 - (1-\frac{1}{n})^n \rightarrow 1 -\frac{1}{e}$ \ARc{Should use different symbols for edges and exponent}.

%We denote the probability space $(\Omega, \mathcal{B}, \mb{P})$ as the domain in which $G$ resides; that is $G: \Omega \rightarrow \lambda(U,V)$ where $\lambda(U,V)$ is the set of all bipartite graphs on $U \times V$. In this way, $G(\omega)$ denotes the (deterministic) graph formed for a particular outcome $\omega \in \Omega$. Similarly, if $N_{v}$ denotes the random neighbourhood of $v \in V$, then $N_{v}(\omega)$ denotes the neighbourhood for the outcome $\omega \in \Omega$. In the remaining subsections, we shall restrict our attention to the case of unit patience; that is, when $\ell_{v}=1$ for all $v \in V$. In addition to non-homogeneous edge probabilities (in contrast to the preceding section), we allow for vertex weights on the offline nodes. We refer to these weights as \textit{rewards}, and denote $w_{u} \ge 0$ as the reward for matching $u$ to an online node of $V$.

%Our main goal in the following sections will be to consider various benchmarks for the instance $G$. Recall that we know that the expected value of the maximum matching is too strong a benchmark to compare probing algorithms against when working with unit patience (the star graph with $p_{e}:=1/n$ for each $e \in U \times V$ is the standard example justifying this). Instead, when comparing the performance of an online probing algorithm on $G$, we take the standard benchmark to be the performance an optimal \textit{offline} probing algorithm. In other words, the adversary is given access to $G$, yet must respect the general constraints of a probing algorithm (decisions on which edges to probe depends on the past history, and the distributional information). It may however adaptively choose the order in which it selects vertices of $V$ to probe, hence the terminology of \textit{offline}. We refer to the value of this benchmark by $\OPT_{off}(G)$ for the instance $G$.


%Another benchmark we consider involves restricting the above class of probing algorithms to ones which are online. In other words, we only consider probing algorithms which respect the online order of $V$ (say $v_{1}, \ldots ,v_{n}$), and define the benchmark to be the maximum expected matching amongst all such algorithms. We denote this benchmark by $OPT_{on}(G)$, and observe that trivially $OPT_{on}(G) \le OPT_{off}(G)$. We also note that since we only care about the performance of online probing algorithms on the specific instance $G$, the adversary may be assumed to have access to the distributional information of $G$.

\ARc{Probably should move the following example to the following section where it is more relevant with the Goyal framework}

\ABc{I agree with Akash and I have inserted the example at the end of what was section 3.1 and now is section 5.1. I didn't delete the example here but will do so once we agree that the new location is where it belongs. 
Do we need another example for arbitrary patience?}

\ARc{We do not need another example for arbitrary patience since negative example for unit patience is still a negative example for arbitrary patience. Also the example should be in section 4 rather than section 5.}

We begin by giving an example where the order of probing edges effect the expected value of matching obtained in case of offline probing algorithms.

\begin{example}
\label{example:order-gap}
Let us consider the bipartite graph $G = (U, V, E)$ where $U = \{u_1, u_2\}$ is the set of offline vertices, $V = \{v_1, v_2\}$ is the set of online vertices and $E = \{(u_1, v_1), (u_2, v_1), (u_2, v_2)\}$ is the set of edges. The edges are stochastic and exists with probabilities $P(u_1, v_1) = \frac1{2}$, $P(u_2, v_1) = 1$ and $P(u_2, v_2) = \frac{1}{2}$. All of these probabilities are independent. The online vertices each have a patience of $1$, whereas the offline nodes have unlimited
patience. In this graph, if edges corresponding to vertex $v_1$ are probed before $v_2$, the expected size of matching is at most 1 while if edges corresponding to vertex $v_2$ are probed before $v_1$, the expected size of matching is $\frac{5}{4}$ for some algorithm.
\end{example}

\begin{proof}
If we probe vertex $v_1$ before vertex $v_2$, we either probe $(u_1, v_1)$ or $(u_2, v_1)$ while probing $v_1$. If we probe the former, the only other edge that we can probe is $(u_2, v_2)$ and the expected number of edges in the matching found is $\frac{1}{2} + \frac{1}{2} = 1$ since both of these edges exist with probability $\frac{1}{2}$. If instead we probe edge $(u_2, v_1)$, then it is always found to exist and there are no more edges that we can probe. This also gives size of matching as $1$. So, the maximum expected number of edges found in a matching when $v_1$ is probed before $v_2$ is 1.

If instead we probe vertex $v_2$ before $v_1$, we probe $(u_2, v_2)$ and it exists with probability $\frac{1}{2}$. If the edge is found to exist, we probe the edge $(u_1, v_1)$ next with exists with probability $\frac{1}{2}$. In these case, expected size of matching is $\frac{3}{2}$. If the edge is not found to exist, we probe the edge $(u_2, v_1)$ with always exists and therefore in this case, the expected size of matching is $1$. Thus, the expected size of matching when $v_2$ is probed before $v_1$ is $\frac{1}{2}\frac{3}{2} + \frac{1}{2}1 = \frac{5}{4}$.
\end{proof}

As we see from this example, there is a gap of at least $\frac{5}{4}$ between optimal probing algorithm in case the order of probing is changed.


==> content/diff-prelim <==
77c77
< between $\OPT(G)$ and $\LPOPT_{old}(G)$ can become quite small, depending on the values of $(\ell_{v})_{v \in V}$
---
> between $\OPT(G)$ and $\LPOPT(G)$ can become quite small, depending on the values of $(\ell_{v})_{v \in V}$
79c79
< as the infinum of this ratio across all stochastic graphs, namely $\inf_{G}\OPT(G)/ \LPOPT_{old}(G)$.
---
> as the infinum of this ratio across all stochastic graphs, namely $\inf_{G}\OPT(G)/ \LPOPT(G)$.
266d265
< 
379a379
> 
484c484
< If that order changes then we can change the order here. Calum: is this the one result where the reult holds wrt the Brubach et al LP?}
---
> If that order changes then we can change the order here.}
496,497c496
< 
< \item Theorem \ref{thm:known-ROM-edge-weights} shows that Algorithm \ref{alg:offline_general_patience} is 
---
> \item Theorem \ref{thm:classical_ROM_greedy} shows that Algorithm \ref{algo:known-rom-edge-weight} is 
499d497
< \ABc{I know that we discussed using Algorithm 3 for both the preceding resul and this result but we really need two Algorithms, one for vertex weight and andversarial order, and one for edge weights and ROMm order. It is indeed the same algorithm and we can perhaps get away with one Algorithm with some explanation and making Algorothm 3 into a template. I am going to try to make it into a template.}
511c509
< \item Theorem \ref{thm:ROM_edge_weights} shows that Algorithm \ref{alg:ROM_edge_weights} is an online algorithm with competitive ratio $\frac{1}{e}$ in the following setting: 
---
> \item Theorem \ref{thm:ROM_edge_weights} shows that Algoirithm \ref{alg:ROM_edge_weights} is an online algorithm with competitive ratio $\frac{1}{e}$ in the following setting: 


==> content/notes7-8 <==
abstract:patience or budget ?  Not timeout



THE PATIENCE CONstraint constraitn results  ....change to  Arbitrary Patience constraints result 

..................


Intro

second paragraph  offline vertices or edges having kopawn  weights and then the objective is to maximize the expected weight of the matching where the expectatgion is with respect the edge probabilities

Notably in Chen et al, the entire ....

Third paragraph     each online vefrtex (and it s adjacent edges) is drawn independently and identically from a known disttribution. That is, in their model ...


In both of these models   In b oth the Chen et al and gthe Bansal et al 

Maybe the last pafragraph of intro becomes first paragraph of section 2
NO leave it where it is


....................

section 2 

  last sentence before subsection 2.1
  following what is standard in ....


secttion 2.1  first paragraphn   In both ....  change to  For both 
          ...  not clear how to compute these optimal benchmark values.  

    Bansal .... of the committal benchmark OPT(G)

   \allaininline{need to state a referenc e for the results against the Bansal LP. } 
   add this at the end of theb  paragrpah before equaltion 2.6


   IN the paragraph  Clearly  on page "for evety vertex of U"
   not sure whyb this is for every vertex.  This isn OK, I misread

   last full paragraoh of page 6   line after (2.7)  probability that a probing
   change the power of the commital benchmark to the  behavior of the commttal benchmartke


   page   comment on what it means to be non-greedy   line 6 after alg 2

  go over Calum's comments at the end of subsection 2.2  need to check appemndix C
   

  in footnote 10, we make a claim re appendix C   need to check


  In subsection 2.3, we should again  comment that ROM does not imply iid in the staochastic setting 
  that is does not follow from Karande et al  It is stated n the intro but worth repeating. 





==> content/summary <==



\subsection{An Overview of Results}

With these definitions in mind and using appropriate LP relaxations of the ideal benchmark, 
we now reiterate and point ahead to our main results as first stated in our abstract. All of our results are competitive ratios against the new LP we introduce.

%\ABc{We  provide Theorem references here corresponding to results as stated in the abstract. I am commenting on the significance/novelty of these results. Check that I have not misstated anything.}  

\begin{enumerate}

\item Theorem \ref{thm:known_vertex_weights} shows that Algorithm \ref{alg:offline_general_patience} is a non-adaptive online  algorithm with competitive ratio $1-\frac{1}{e}$ in the following stochastic setting:

\begin{itemize}

\item There is a known stochastic graph
\item Online vertices are given adversarially, and have an arbitrary patience parameter, and offline vertices have weights.  
\end{itemize}
This result shows that the .544 inapproximation bound against $LPOPT_{old}$ does not hold wrt our benchmark. \ARc{Do we mention here that it also does not hold wrt the Bruback et al LP. I think we can mention when we state/discuss ROM result in the unknown graph setting}.

\item Theorem \ref{thm:known-ROM-edge-weights} shows that Algorithm \ref{alg:offline_general_patience} is 
an online algorithm with competitive ratio $\frac{1}{2}$ in the following setting:

\begin{itemize}
\item There is a known stochastic graph
\item Online vertices are presented in an order determnined by a uniform at random permutation of the online vertices in the stochastic graph (i.e., stochastic ROM model) 
\item Online vertices have arbitrary patience
\item Edges have weights

\end{itemize}

We note that this result and the previous result are derived from the same algorithm; the difference between this result and the previous result is that here we consider edge weights and ROM input sequences and hence this result is incomparable with the previous result.

%\ABc{We note that previous results for the stochastic rewards and ROM arrivals are immediate consequences of the corresponding result for This is a result in a setting (e.g., edge weights) not previously studied.} 

\item \ABc{Waiting to see how we organize the statement of results for the unknown stochastic graph setting when we have three specific results. We do not have an explicit Theorem to refer to. Here is what I think we want to say: Following the Devanur et al \cite{DJK2013} primal dual analysis for unweighted and vertex weighted bipartite matching in the classical (ie.e, non-stochastic) setting, the development in Section \ref{sec:rom-model} provides a {\it deterministic} algorithm for stochastic rewards wth ROM arrivals. The algorithm does not know the stochastic graph. As a consequence, we are showing that the $1-\frac{1}{e}$ competitive ratio for vertex weighted bipartite matching can be acheived by a deterministic ROM algorithm whereas this bound was previously only known for randomized algorithms albeit with adversarial inputs. Unlike the unweighted case, there is no immediate duality bewteen the two vertex weighted settings.}  

\item Theorem \ref{thm:ROM_edge_weights} shows that Algorithm \ref{alg:ROM_edge_weights} is an online algorithm with competitive ratio $\frac{1}{e}$ in the following setting: 

\begin{itemize}
\item The stochastic graph is not known to the algorithm
\item Online vertices are presented in an order determnined by a uniform at random permutation of the online vertices in the stochastic graph (i.e., stochastic ROM model)
\item Online vertices have unit patience
\item Edges have weights

\end{itemize}
This generalizes the classical non stochastic result of Kesselheim \cite{edgeweightedrom}.

\item Theorem \ref{thm:iid} shows that Algorithm \ref{alg:known_iid} is a
non-adaptive online algorithm with competitive ratio $1-\frac{1}{e}$ in the following stochasic i.i.d. setting:

\begin{itemize}
\item There is a known stochastic (type) graph
\item Online vertices are drawn independently and identically from a distibution on the vertices (with their adjacent stochastic edges)
\item Online vertices have arbitrary patience
\item Edges have weights

\end{itemize} 




==> content/temp <==
new_LP_relaxations.log:\citation{edgeweightedrom}
new_LP_relaxations.log:l.1333 ...ult of Kesselheim \cite{edgeweightedrom}
new_LP_relaxations.log:LaTeX Warning: Citation `edgeweightedrom' on page  undefined on input line 1333
prelim.log:\citation{edgeweightedrom}
prelim.log:l.485 ...sult of Kesselheim \cite{edgeweightedrom}
prelim.log:LaTeX Warning: Citation `edgeweightedrom' on page  undefined on input line 485.
prelim.tex:%This generalizes the classical non stochastic result of Kesselheim \cite{edgeweightedrom}.
summary:This generalizes the classical non stochastic result of Kesselheim \cite{edgeweightedrom}.


==> content/temp-unknown <==

\item 


%Waiting to see how we organize the statement of results for the unknown stochastic graph setting when we have three specific results. We do not have an explicit Theorem to refer to. Here is what I think we want to say: 
Following the Devanur et al. \cite{DJK2013} primal-dual analysis for unweighted and vertex weighted bipartite matching in the classical (i.e, non-stochastic) setting, the development in Section \ref{sec:online-rom} provides a {\it deterministic} algorithm for online stochastic matching with ROM arrivals. Theorem \ref{thm:unknown-special-cases} shows that when the stochastic graph is not known, there is a deterministic online algorithm that obtains a $1-\frac{1}{e}$ competitive ratio  for any of the following special cases:

%\CMc{Mention that our result for unit patience shows that an analogous hardness result
%of that of Mehta \cite{MehtaP12} (unit patience, adversarial arrivals, against Bansal LP) does not apply.
%Also, mention that we can follow the primal dual charging argument of Devanur, whereas more complicated
%techniques are needed in the adversarial order model, as seen recently in \cite{huang2020online}. Results
%are surprising, since there is an equivalence between ROM and deterministic algorithms/ Adversarial and randomized algorithms, as we review and generalize in the Appendix.}


\begin{itemize}
	\item When the offline vertices are unweighted; i.e., $w_u = 1$ for each $u \in U$
    \item When the edge probabilities are \textit{online vertex uniform};  i.e., for each $v \in V$, there exists
    $p_v$ such that $p_{u, v} = p_v$ for all $u \in N(v)$
    \item When the patience of each online vertex is $1$
\end{itemize}

We note that Brubach et al. \cite{Brubach2019} observe that $.544$ is  the best possible competitive ratio against the Bansal et al. LP
for full patience ($\ell_v = |U|$ for all $v \in V$). Their example for the inapproximation applies to the special case that all online nodes are identical and hence the inapproximation applies to the ROM, known stochastic graph, and the stochastic i.i.d. settings. They speculate that the .544 inapproximation can be overcome for arbitrary patience in the unknown adversarial stochastic matching model, by looking at a new LP relaxation that they define. In the ROM model, our result lends some support to their conjecture, as we show that the Brubach et al. algorithm obtains a competitive ratio of $1-\frac{1}{e}$ in this setting. As a further observation, in the case of unit patience, we contrast our ROM result with the recent results for stochastic matching in Huang and Zhang 
\cite{huang2020online}. They discuss the difficulty to date in applying the 
primal-dual argument of Devanur et al. to achieve a competitive ratio greater than $.5$ (obtained by a greedy algorithm).  For  unit patience they are able to  show a randomized $.572$ competitive ratio for adversarial online inputs when edge probabilities are vanishing. 
Finally, with respect to our ROM result in the case of unit patience, we emphasize that the randomized $.621 < 1-\frac{1}{e}$ inapproximation %\CMc{Perhaps reword this} 
in Mehta and Panigraphi \cite{MehtaP12} is with regard to  the adversarial input model and applies to any of the LPs discussed in this paper (since it is for the unit patience case). Our result shows that this inapproximation cannot apply to the ROM input model.  


